The Devil is in the Tails: How Long-Tailed Code Distributions Impact Large Language Models

Learning-based techniques, especially advanced Large Language Models (LLMs) for code, have gained considerable popularity in various software engineering (SE) tasks. However, most existing works focus on designing better learning-based models and pay less attention to the properties of datasets. Learning-based models, including popular LLMs for code, heavily rely on data, and the data's properties (e.g., data distribution) could significantly affect their behavior. We conducted an exploratory study on the distribution of SE data and found that such data usually follows a skewed distribution (i.e., long-tailed distribution) where a small number of classes have an extensive collection of samples, while a large number of classes have very few samples. We investigate three distinct SE tasks and analyze the impacts of long-tailed distribution on the performance of LLMs for code. Our experimental results reveal that the long-tailed distribution has a substantial impact on the effectiveness of LLMs for code. Specifically, LLMs for code perform between 30.0\% and 254.0\% worse on data samples associated with infrequent labels compared to data samples of frequent labels. Our study provides a better understanding of the effects of long-tailed distributions on popular LLMs for code and insights for the future development of SE automation.

==> Sections/Method.tex <==
\section{Long-tailed Code Distribution}


\noindent\textbf{Code Distribution.}
Following the definition of image distribution in the computer vision domain where researchers have actively studied the long-tailed distributions in images for a decade~\cite{liu2019large,yang2022survey_lt,focal,cb,bs,wei2021crest},  the code distribution is formulated as below:
\begin{equation}
D(x_i) \sim P(y_i) = freq(y_i) 
\end{equation}
where $freq(y_i)$ is the frequency of samples belonging to class $y_i$ in the data.

In the context of multi-class classification tasks in software engineering, calculating the frequency of each class is straightforward since the labels (ground truths) directly represent the corresponding classes.

However, for generation-based tasks, the labels are sequences of tokens with potentially different meanings across different tasks. Therefore, it is necessary to customize the computation of label frequencies based on the task's specific goals. For API sequence recommendation, the aim is to recommend \textit{a sequence of APIs}, with a single API being the basic component.
In this case, each target API is treated as a separate label, and the frequency of each API in the dataset is calculated as $Pa(API_i) = freq ( API_i ).$
Given an input sample $x_i$ with the ground truth label $y_i = [API_1, API_2, API_3, ..., API_k]$, we define the $freq(y_i)$ by averaging the frequencies of each API in $y_i$.
\begin{equation}
D(x_i) \sim P(y_i) = freq(y_i) = \frac{\sum_{API_i \in y_i} Pa(API_i)}{k}
\end{equation}

For code revision recommendations, the aim is to suggest \textit{code modifications} that enhance the quality of the submitted code towards the accepted code by reviewers. Therefore, only the changed code tokens (e.g., newly added, replaced, deleted) are relevant, and not all code tokens in the ground truth (i.e., the accepted version of code). In this case, we consider each token-level edit as one label and compute the frequencies of edits in the entire dataset. An edit is defined as a pair of code tokens $\langle$token before, token after$\rangle$. For instance, if the action is ``add'', then the ``token before'' will be an empty string, and the ``token after'' will be the newly added token.
The edit distribution is represented as $Pe(edit_i) = freq ( edit_i ).$ Given an input $x_i$ with a ground truth $y_i = [edit_1, edit_2, edit_3, ..., edit_k]$, we calculate $freq(y_i)$ by averaging the frequencies of each edit in $y_i$:
\begin{equation}
D(x_i) \sim P(y_i) = freq(y_i) = \frac{\sum_{edit_i \in y_i} Pe(edit_i)}{k}
\end{equation}





\vspace{0.1cm}
\noindent\textbf{Head and Tail Data.}
In this work, we define that a code dataset holds up the long-tailed distribution if a small portion of classes (head classes) have massive sample points while some other classes (tail classes) have very few data samples.
To understand the impact of the long-tailed distribution, we split a dataset \emph{evenly} into two parts. 
\begin{enumerate}[leftmargin=*]
\item \textit{\textbf{Head data:}} 
This 50\% of the data samples are selected from the classes that contain the largest number of samples. 
\item \textit{\textbf{Tail data:}}
On the contrary, this 50\% of the data samples are taken from the classes that include the lowest number of samples. 
\end{enumerate}
Please note that the tail data has the same number of samples as the head data, while tail data consists of a large number of classes, and samples for each class are relatively few.





 
\noindent\textbf{Characterizing Long-tailedness in Datasets.} 
Accurate measurement of the long-tailedness of data is an important aspect of understanding the dataset~\cite{yang2022survey_lt}. 
In this work, we adopt the Gini Coefficient~\cite{gini1912variabilit} as the metric to quantify the long-tailedness.
The Gini Coefficient is recommended as the ideal metric by a systematic survey~\cite{yang2022survey_lt} of long-tailed distribution studies since it is neither affected by extreme samples nor the absolute number of data as well as it is bounded from 0 to 1.


We denote $x_i$ as the number of data samples belonging to the class $i$ and there are $n$ classes in total.
The Gini coefficient is defined as half of the relative mean absolute difference~\cite{gini1912variabilit,sen1997economic}. The mean absolute difference is the average absolute difference in terms of the number of samples for all pairs of classes in the distribution, and the relative mean absolute difference is the mean absolute difference divided by the average number of samples for all classes ($\bar x = \frac{\sum_{i=1}^{n} x_i}{n}$), to normalize for scale. Formally, the Gini coefficient is given by:
\begin{equation}
Gini = \frac{1}{2} \underbrace{\underbrace{\frac{ \sum_{i=1}^{n} \sum_{j=1}^{n} |x_i - x_j| }{ \sum_{i=1}^{n} \sum_{j=1}^{n} 1}}_{\text{mean absolute difference}}  \frac{1}{\bar x}}_{\text{relative mean absolute difference}}
\\
= \frac{\sum_{i=1}^{n} \sum_{j=1}^{n} |x_i - x_j|}{2n^2 \bar x}
\end{equation}
Please note that a Gini coefficient of 0\% indicates perfect equality where every class has the same number of data samples, while a Gini coefficient of 100\% expresses full inequality where only one class has all the data points. The higher the Gini coefficient is, the heavier the long-tailed distribution is. 


==> latex_util.tex <==
\newcommand{\basicalert}[2]{\fbox{\bfseries\sffamily\scriptsize\color{blue} #1}{\sf\small$\blacktriangleright$\textit{\color{red} #2}$\blacktriangleleft$}}
\newcommand{\bowen}[1]{\basicalert{From Bowen}{#1}}


% \newcommand{\toolname}{\mbox{CCBERT}\xspace}
